Scenario-Based Field Testing of Drone Missions

Testing and validating Cyber-Physical Systems (CPSs) in the aerospace domain, such as field testing of drone rescue missions, poses challenges due to volatile mission environments, such as weather conditions. While testing processes and methodologies are well established, structured guidance and execution support for field tests are still weak. This paper identifies requirements for field testing of drone missions, and introduces the Field Testing Scenario Management (FiTS) approach for adaptive field testing guidance. FiTS aims to provide sufficient guidance for field testers as a foundation for efficient data collection to facilitate quality assurance and iterative improvement of field tests and CPSs. FiTS shall leverage concepts from scenario-based requirements engineering and Behavior-Driven Development to define structured and reusable test scenarios, with dedicated tasks and responsibilities for role-specific guidance. We evaluate FiTS by (i) applying it to three use cases for a search-and-rescue drone application to demonstrate feasibility and (ii) interviews with experienced drone developers to assess its usefulness and collect further requirements. The study results indicate FiTS to be feasible and useful to facilitate drone field testing and data analysis

==> _format.tex <==
\usepackage{fancyhdr}
\usepackage{amsthm}%
\usepackage{mathrsfs}%
\usepackage[title]{appendix}%
\usepackage{manyfoot}%
\usepackage{algorithm}%
\usepackage{algorithmicx}%
\usepackage{algpseudocode}%
\usepackage{listings}%
\usepackage{amsmath,amssymb,amsfonts} %%assymb breaks the acm template
\usepackage{url}
\usepackage{booktabs} % For formal tables                  
%\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{xspace}
\usepackage{hyperref}
\usepackage{balance}
\usepackage{tabularx}

\usepackage{booktabs}
\usepackage{multicol}
\usepackage{multirow}
\usepackage{rotating}
\usepackage{caption}
%\usepackage{subfigure}
\usepackage{subcaption}
\usepackage[export]{adjustbox}
\usepackage{tabularx}
\usepackage{tikz}
\usepackage{float}
\usepackage[shortlabels]{enumitem}
\usepackage[font=small]{caption}

\usepackage{wasysym}

\usepackage{csquotes}
\MakeOuterQuote{"}

\definecolor{commentGreen}{RGB}{128,127,41}
\definecolor{stringGreen}{RGB}{0,127,38}
\definecolor{keywordRed}{RGB}{151,0,11}
\definecolor{typePurple}{RGB}{128,3,82}
\definecolor{variableBlue}{RGB}{0,0,255}
\definecolor{annotationRed}{RGB}{198,4,38}
\definecolor{annotationBlue}{RGB}{32,21,223}

\newcommand{\etal}[1][]{%
\ifthenelse{\equal{#1}{}}{\emph{et~al.}\xspace}{\emph{et~al.}~\cite{#1}\xspace}%
}

\newcommand{\citesec}[1]{Section~\ref{sec:#1}}
\newcommand{\citefig}[1]{Fig.~\ref{fig:#1}}
\newcommand{\citealgo}[1]{\textsc{Listing}~\ref{algo:#1}}
\newcommand{\citelisting}[1]{\textsc{Listing}~\ref{lst:#1}}
\newcommand{\citetable}[1]{{Table}~\ref{tab:#1}}
\newcommand{\citedef}[1]{\textsc{Definition}~\ref{def:#1}}
\newcommand{\citesecs}[2]{Sections~\ref{sec:#1} and~\ref{sec:#2}}

% \newcommand{\mv}[1]{{\textcolor{orange}{#1}}}%orange
% \newcommand{\ig}[1]{{\textcolor{blue}{#1}}}%blue
% \newcommand{\ta}[1]{{\textcolor{green}{#1}}}%green

% \newcommand{\fwname}{{\textcolor{purple} EduComp}\xspace}%orange


\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash}p{#1}} 
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash}p{#1}} 
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash}p{#1}} 


\newcommand{\bullitem}[1]{\noindent$\bullet$\textbf{ #1}}

\newcommand{\intqte}[1]{\emph{#1}}

